Addressing Cold Start in Recommender Systems with Hierarchical Graph Neural Networks

Recommender systems have become an essential instrument in a wide range of industries to personalize the user experience. A significant issue that has captured both researchers' and industry experts' attention is the cold start problem for new items. In this work, we present a graph neural network recommender system using item hierarchy graphs and a bespoke architecture to handle the cold start case for items. The experimental study on multiple datasets and millions of users and interactions indicates that our method achieves better forecasting quality than the state-of-the-art with a comparable computational time.

==> author.tex <==
\author{Ivan Masimov$^{1}$, Rodrigo Rivera-Castro$^{1}$ and Evgeny Burnaev$^{1}$% <-this % stops a space
\thanks{Sections I, II, III, IV were supported by the Ministry of Education  and  Science  of  the  Russian  Federation  (Grant no. 14.756.31.0001). Other sections were supported by the Mexican National Council for Science and Technology (CONACYT), 2018-000009-01EXTF-00154.}% <-this % stops a space
\thanks{$^{1}$Skoltech, Moscow, Russia
        {\tt\small ivan.maksimov at skoltech.ru}}%

}
